Partial End-to-end Reinforcement Learning for Robustness Against Modelling Error in Autonomous Racing

In this paper, we address the issue of increasing the performance of reinforcement learning (RL) solutions for autonomous racing cars when navigating under conditions where practical vehicle modelling errors (commonly known as \emph{model mismatches}) are present. To address this challenge, we propose a partial end-to-end algorithm that decouples the planning and control tasks. Within this framework, an RL agent generates a trajectory comprising a path and velocity, which is subsequently tracked using a pure pursuit steering controller and a proportional velocity controller, respectively. In contrast, many current learning-based (i.e., reinforcement and imitation learning) algorithms utilise an end-to-end approach whereby a deep neural network directly maps from sensor data to control commands. By leveraging the robustness of a classical controller, our partial end-to-end driving algorithm exhibits better robustness towards model mismatches than standard end-to-end algorithms.

==> Figures/EndToEndAlgorithm/ete_hyperparams.tex <==
\newcolumntype{R}{>{\raggedleft\arraybackslash}p{4cm}}
\newcolumntype{C}{>{\raggedright\arraybackslash}p{1.5cm}}
\newcolumntype{L}{>{\raggedright\arraybackslash}p{1.5cm}}

\begin{table}[htb!]
\centering
%\renewcommand{\arraystretch}{1.1}
\small
\begin{tabularx}{\columnwidth}{RCL} 
    \hline
    \textbf{Hyper-parameter} & \textbf{Symbol} & \textbf{Value} \\ 
    \hline
    \textbf{Algorithm}                      & $1.5 \cdot 10^5$          & \\
    Maximum time steps                      & $M$                       &  \\
    Target update rate                      & $\tau$                    & $5\cdot10^{-3}$ \\
    Replay buffer size                      & $\mathcal{B}$             & $5\cdot 10^5$ \\
    Replay batch size                       & $B$                       & $400$ \\
    Exploration noise standard deviation    & $\sigma_{\text{action}}$  & $0.1$ \\
    Reward discount rate                    & $\gamma$                  & $0.99$ \\
    Agent samples between network updates   & $d$                       & $2$ \\
    Agent sample rate                       & $f_{\text{agent}}$        & $5$ Hz \\
    Target action noise standard deviation  & $\tilde{\sigma}$          & $0.2$ \\ 
    Target action noise clip                & $c$                       & $0.5$ \\
    \textbf{Reward signal}                  &                           & \\
    Distance reward                         & $r_{\text{dist}}$         & $0.25$ \\ 
    Time step penalty                       & $r_{\text{time}}$         & $0.01$ \\
    Collision penalty                       & $r_{\text{collision}}$    & $-10$ \\
    \textbf{Observation}                    &                           & \\
    Number of LiDAR beams                   & L                         & 20 \\
    % Observation noise                       & $\sigma_{\text{observation}}$ & $x=0.025$ m, $y=0.025$ m, $\theta=0.05$ rads, $v=0.1$ m/s, $\text{LiDAR distances}=0.01$ m \\                      
    \textbf{Neural network}                 &                           & \\
    Learning rate                           & $\alpha$                  & $10^{-3}$ \\
    Neurons in input layer                  & $m_1$                     & 400 \\
    Neurons in hidden layer                 & $m_2$                     & 300 \\
    \textbf{Velocity constraints}           &                           & \\
    Minimum velocity                        & $v_{\text{min}}$          & $3$ m/s \\
    Maximum velocity                        & $v_{\text{max}}$          & $5$ m/s \\
    \hline
\end{tabularx}
\caption[Selected values of hyper-parameters for the end-to-end algorithm]{Selected values of hyper-parameters for the end-to-end racing algorithm on the Porto track.}
\label{tab:eteHyperparams}
\end{table}


==> Figures/EndToEndAlgorithm/reward_signal.tex <==
\newcolumntype{R}{>{\raggedleft\arraybackslash}p{4cm}}
\newcolumntype{C}{>{\centering\arraybackslash}p{1.5cm}}
\newcolumntype{L}{>{\raggedright\arraybackslash}p{1.5cm}}

\begin{table*}[htb!]
\centering
\renewcommand{\arraystretch}{1.5}
\small
\begin{tabularx}{\textwidth}{RCCCCCCC} 
    \hline
     & & \multicolumn{3}{c}{\textbf{End-to-end}} & \multicolumn{3}{c}{\textbf{Partial end-to-end}} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8} 
    \textbf{Reward signal component} & \textbf{Symbol} & \textbf{Porto} & \textbf{Barcelona-Catalunya} & \textbf{Monaco} & \textbf{Porto}  & \textbf{Barcelona-Catalunya}  & \textbf{Monaco} \\ 
    \cmidrule(lr){1-2} \cmidrule(lr){3-8} 
    Distance reward                         & $r_{\text{dist}}$         & $0.25$ & $0.3$ & $0.3$ & $0.2$ & $0.2$ & $0.25$ \\ 
    Time step penalty                       & $r_{\text{time}}$         & $-0.01$ & $-0.01$ & $-0.01$ & $-0.01$ &  $-0.01$ & $-0.01$ \\
    Collision penalty                       & $r_{\text{collision}}$    & $-10$  & $-2$ & $-2$ & $-5$ &  $-5$ & $-5$ \\
    \hline
\end{tabularx}
\caption{values of reward signal components for each algorithm and track that resulted in optimal performance.}
\label{tab:rewardSignal}
\end{table*}


==> Figures/RelatedWork/partial_end_to_end_learned_control.tex <==
% \tikzstyle{a}=[rectangle, draw=black, fill=white,thick, minimum width = 2cm, minimum height = 3cm, align=center, rounded corners=.1cm, font=\small]
\tikzstyle{b} = [rectangle, draw=black, fill=white,thick, minimum width = 2cm, minimum height = 1cm, align=center, rounded corners=.1cm, font=\normalsize,  align=center]
\tikzstyle{c} = [shape aspect=1, circle, minimum width=1.8mm, draw=black, inner sep=0pt]


\begin{tikzpicture}
 
    % Draw nodes
    \node (a) at (0,0)      [b, fill=gray!20] {Sensors};
    \node (left) at (2.5,0)    [b] {Perception};
    \node(center) at (5,0)  [] {};
    \node (c) at ($(center)+(2.5,0)$) [] {};
    \node (d) at ($(center)+(0,0)$) [b] {Planner};
    \node (right) at (7.5,0)    [] {};
    \node (e) at (10,0)     [b, fill=gray!20] {Actuators};

    

    %Draw neural network
    \node (nnl1r1) at ($(c)+(-0.5,0.4)$) [c] {};
    \node (nnl1r2) at ($(c)+(-0.5,0)$) [c] {};
    \node (nnl1r3) at ($(c)+(-0.5,-0.4)$) [c] {};
    
    \node (nnl2r1) at ($(c)+(0,0.4)$) [c, label={[align=center]\footnotesize Learned\\controller}] {};
    \node (nnl2r2) at ($(c)+(0,0)$) [c] {};
    \node (nnl2r3) at ($(c)+(0,-0.4)$) [c] {};
    \node (nnl3r1) at ($(c)+(0.5,0.2)$) [c] {};
    \node (nnl3r2) at ($(c)+(0.5,-0.2)$) [c] {};

    
    
    % Draw boxes around nodes
    % Driving architecture
    \draw[loosely dashed] ($(left)+(-1.25,-0.8)$) -| ($(right)+(1.25,1.6)$) -|  ($(left)+(-1.25,-0.8)$);
    
    % Draw connections
    \draw[->] (a) -- (left);
    \draw[->] (left) -- (d);
    \draw[->] (d) -- (nnl1r2);
    \draw[->] ($(c)+(0.6,0)$) -- (e);

    
    \draw[->] (nnl1r1) -- (nnl2r1);
    \draw[->] (nnl1r1) -- (nnl2r2);
    \draw[->] (nnl1r1) -- (nnl2r3);

    \draw[->] (nnl1r2) -- (nnl2r1);
    \draw[->] (nnl1r2) -- (nnl2r2);
    \draw[->] (nnl1r2) -- (nnl2r3);

    \draw[->] (nnl1r3) -- (nnl2r1);
    \draw[->] (nnl1r3) -- (nnl2r2);
    \draw[->] (nnl1r3) -- (nnl2r3);

    \draw[->] (nnl2r1) -- (nnl3r1);
    \draw[->] (nnl2r1) -- (nnl3r2);
    
    \draw[->] (nnl2r2) -- (nnl3r1);
    \draw[->] (nnl2r2) -- (nnl3r2);

    \draw[->] (nnl2r3) -- (nnl3r1);
    \draw[->] (nnl2r3) -- (nnl3r2);
    
\end{tikzpicture}
